HiTailor: Interactive Transformation and Visualization for Hierarchical Tabular Data

Tabular visualization techniques integrate visual representations with tabular data to avoid additional cognitive load caused by splitting users' attention. However, most of the existing studies focus on simple flat tables instead of hierarchical tables, whose complex structure limits the expressiveness of visualization results and affects users' efficiency in visualization construction. We present HiTailor, a technique for presenting and exploring hierarchical tables. HiTailor constructs an abstract model, which defines row/column headings as biclustering and hierarchical structures. Based on our abstract model, we identify three pairs of operators, Swap/Transpose, ToStacked/ToLinear, Fold/Unfold, for transformations of hierarchical tables to support users' comprehensive explorations. After transformation, users can specify a cell or block of interest in hierarchical tables as a TableUnit for visualization, and HiTailor recommends other related TableUnits according to the abstract model using different mechanisms. We demonstrate the usability of the HiTailor system through a comparative study and a case study with domain experts, showing that HiTailor can present and explore hierarchical tables from different viewpoints. HiTailor is available at https://github.com/bitvis2021/HiTailor.

==> 5-2usabilitystudy.tex <==
\subsection{Usability Study}
\label{sec:usability-study}
We conducted a usability study to evaluate the effectiveness of the HiTailor system. Our overall goal is to investigate: (1) whether HiTailor helps users create meaningful visualizations and conduct data analysis; (2) whether the transformations, recommendations and visualization results assist users in exploring the hierarchical tables.

\subsubsection{Study Design}
Based on the above goals, we conducted a formal study to gain insights from ordinary users and understand HiTailor’s usage and limitations.

\textbf{Participants and Apparatus.} 
We recruited 25 participants, including 8 females and 17 males. All of them were undergraduate or postgraduate students with different majors, ranging from computer science to mathematics and statistics, \add{and they often use table to organize and analyze data in their practical applications}. \comment{their background may introduce a bias, need a discussion about it}
We asked participants to specify their experience in using data visualization tools (e.g., PowerBI, Tableau, Matplotlib), where 1-point means ``never heard of it", and 5-point means ``extremely familiar". The average result based on responses from all participants was 3.02 ($\sigma=0.75$).
% \lgz{the programming background?}
% \lrf{Following apparatus need to be changed.maybe not changed} 
The usability test was performed in a quiet computer lab on a Dell Precision T5500 desktop PC, with an Intel Xeon Quad-Core processor, 8GB RAM, and an Nvidia Quadro 2000 graphics card driving a 23-inch LCD 1920 $\times$ 1080 pixel monitor.

\textbf{Dataset.} To better verify the effectiveness of HiTailor, we selected some hierarchical tables from different fields in real-world applications, including sales records, investment analysis, etc. The largest hierarchical table in the dataset consists of 42 rows and 39 columns, while the smallest tabular data has 19 rows and 17 columns. \add{The levels of the row and column headings range from two to three.} \remove{, which had an appropriate complexity for user studies.} 

\textbf{Procedures.} A study session lasted around 60 minutes. First, we provided a tutorial on HiTailor, including the functionalities of different transformation operators and the interaction techniques when authoring tabular visualizations. 
% We also explain the background of target hierarchical tables for subjects. 
After that, we asked the participants to explore the hierarchical table freely using the HiTailor system. 
Users could record their findings by exporting the visualization results into static figures. 
During the usability study, we encouraged participants to think aloud and ask questions.
At the end of the experiment, we asked the participants to rate HiTailor from different aspects using a five-point Likert scale. 
We also conducted a follow-up interview for the participants for about 20 minutes to collect their feedback on HiTailor. During the interview, the participants were encouraged to comment on any aspect of HiTailor, and we would make detailed records.

\begin{figure}[tb]
 \centering
 \includegraphics[width=1\columnwidth]{pictures/usability-result.eps}
 \caption{Ratings from different aspects of HiTailor on a five-point Likert scale (N = 25). The rightmost column indicates the average and standard deviations.}
 \label{fig:usability-result}
\end{figure}

\subsubsection{Participant Feedback}
% Overall, HiTailor received enthusiastic reviews from all the participants. As shown in Fig.~\ref{fig:usability-result}, participants, in general, deemed that HiTailor could help create satisfactory visualizations and facilitate the understanding of hierarchical tabular data. In the following text, we summarized participants’ feedback of HiTailor during the interview.
HiTailor received positive feedback from the participants. As shown in Fig.~\ref{fig:usability-result}, participants generally deemed that HiTailor could help create satisfactory visualizations and facilitate the understanding of hierarchical tabular data. We summarized participants’ feedback on HiTailor during the interview as followings.

\textbf{HiTailor is easy to learn and use.} As a visualization authoring tool, HiTailor scored a high rating among participants in ease of learning ($\mu=4.12,~\sigma=0.77$) and ease of using ($\mu=4.24,~\sigma=0.81$). Some participants emphasized that HiTailor has a short learning curve: \emph{``it was quite easy to get started"} (P8, 14).

\textbf{HiTailor facilitates the creation of various visualizations flexibly.} Several participants commented that HiTailor supported a wide range of visualizations (P3, 9, 23) and intuitive visual mapping (P11). They appreciated the various transformations of hierarchical tabular data, the most impressive of which was \emph{swap} (P1, 6, 15, 16) because of its helpfulness in modifying the positions of data items to create their target visualizations. TableUnit recommendations were also considered useful because it improves the efficiency of the exploration process (P6). \emph{``The recommendation was great! I didn't need to specify the same visualization configurations over and over again."} (P20).

\textbf{HiTailor supports impressive interactive exploration.} Several participants enjoy the user experience of HiTailor, especially highlighting the corresponding headings when hovering over visualizations (P3, 24). \emph{``The highlighting kept me from switching back and forth between visualizations and original data values."} (P19). Many participants commented on the legends and tooltips of visualizations as helpful, but some indicated that some legends were imperfect and not easy to understand (P2, 5). After analyzing this problem, we found that it was partly due to the limitations of Vega-Lite, which we would consider optimizing in future work.

% show a tabular data for users, using excel and HiTailor. comparing the insights from the tabular data. 
% \begin{equation}
% \sum_{j=1}^{z} j = \frac{z(z+1)}{2}
% \end{equation}

==> README <==
Created by Torsten Moeller (vis@cs.sfu.ca), April 6 2004
modified by Steven Bergner and Torsten Moeller, June 30 2006
modified by James Peltier and Torsten Moeller, March 28, 2007
modified by Bernhard Finkbeiner, July 5, 2010
modified by Tobias Isenberg, January 2016
modified by Filip Sadlo, March 2016
modified by Tobias Isenberg, July 2016

This distribution provides a document class for formatting papers according to the specifications for submission to conferences sponsored by the IEEE Visualization & Graphics Technical Committee (VGTC).

Conferences that use the 'journal' document option:
- IEEE Visualization Conference (VIS, incl. InfoVis, SciVis, VAST)
- IEEE Virtual Reality (VR)
- IEEE International Symposium on Mixed and Augmented Reality (ISMAR)

It contains 13 files/directories:

README          - this file
diamondrule.eps - abstract and body separator
diamondrule.pdf - its PDF version
vgtc.cls        - the VGTC class file, which should be placed, somewhere in the TeX search path (or in the local directory)
template.tex    - an example paper
template.bib    - a small bibliography file used by the example
template.pdf    - an example proper pdf output in default journal mode
abbrv-doi*.bst  - four different versions to generate the bibliography including DOI output, with and without hyperref support, with and without narrow rendering of DOIs
makefile        - makefile including bibtex compilation and proper PDF generation
pictures/       - subdirectory with sample images, both in EPS and in direct pixel/vector format

Usage
=====

The template can be used as such (using the established LaTeX environments) by calling pdfLaTeX or LaTex. For Windows-based LaTeX installations you can use, for example, the environment provided by http://www.texniccenter.org/ along with MikTeX (http://miktex.org/). For Uinux-based installations, please use your favorite LaTeX distribution and editing environment or use the makefile following the instructions below.

Use of the Makefile
===================

Prior to "building" a paper please be sure to run

  make clean

This will ensure that the paper is built cleanly each and every time. We suggest to run this command before each new compilation.

To compile the example, run

  make

or manually, if the makefile does not work for you

  latex template
  bibtex template
  latex template
  latex template

If you run 'make' for the first time, a successful compilation will create a file called 'template.pdf'. Please make sure, that its layout is identical to the file 'template-journal.pdf' provided with this package.

The included makefile also allows you to run each step of the process manually.  Below are a list of available options that may be passed to make

 "make clean"
   removes all files that can be generated automatically.

 "make gs7"
   This will perform all functions to build a proper paper using GhostScript 7.

 "make gs8"
   This will perform all functions to build a proper paper using GhostScript 8.

 "make dvi"
   This will process the .tex file and produce a DVI output file.  This
   step may process the .tex file several times to process all references
   and citations.

 "make ps"
   This will process the .tex file and the DVI output and convert it to a
   PostScript file.

 "make pdf"
   This will process the .tex file using pdfTeX/pdflatex to produce a PDF
   file directly (not using a DVI and PostScript file).
   Please make sure that all fonts are embedded.
   You can use pdffonts my_document.pdf to check if they are.
   It is standard in all modern latex distributions.
   If you use eps figures (e.g. R or gnuplot figures) which you convert to
   PDF using epstopdf, do the following:
   Use GL_OPTIONS, a global environment variable for ghostscript:
   export GS_OPTIONS="-dEmbedAllFonts=true -dPDFSETTINGS=/printer"
   # and run
   epstopdf myfile.eps

   See http://bugs.debian.org/cgi-bin/bugreport.cgi?bug=411651 for the
   origin of this solution.


If you have problems with the makefile please notify us with the output of
the errors produced when running make and we will work to figure out the
resolution.


To produce proper pdf output, please use:
  dvips -t letter -Pdownload35 -Ppdf -G0 template.dvi -o template.ps

The "-Ppdf" and "-G0" flags should be specified in that order; reversing
them does not work, and will result in unacceptable results.

The following information is an exerpt from the ACM SIGGRAPH Conference /
Symposium / Workshop Content Formatting Instructions which can be found
here.

 http://www.siggraph.org/publications/instructions/author-instructions.pdf

If you are using version 7.x of GhostScript, please use the following
method of invoking ‘ps2pdf,’ in order to embed all typefaces and ensure
that images are not downsampled or subsampled in the PDF creation process:

 ps2pdf -dCompatibilityLevel=1.3 -dMaxSubsetPct=100 \
        -dSubsetFonts=true -dEmbedAllFonts=true \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

If you are using version 8.x of GhostScript, please use this method in
place of the example above:

 ps2pdf -dPDFSETTINGS=/prepress -dCompatibilityLevel=1.3 \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

This has been incorporated into the makefile and should no longer be needed
unless you are building the PDF file manually.


==> makefile <==
# This file seems to originate from something called 'the ultimate
# latex makefile' that different authors worked on. Find original
# versions at:
# http://tadek.pietraszek.org/blog/2006/03/24/the-ultimate-latex-makefile/
# (c) by Tadeusz Pietraszek
# http://www.acoustics.hut.fi/u/mairas/UltimateLatexMakefile/ 
# (c) by Matti Airas
#
# This file has been assembled and adjusted by Steven Bergner, Nov 2005
#  - support for multiple sub-texfiles
#  - fixed '=' '#' problem in mingw/msys environment (see E variable)
#  - PS compilation uses VGTC recommended settings
#  - targets restructured to make PDF by default
#
# Call 'make dvi' for minimal compilation, to check for proper latex
# syntax. This can be much faster than a full PDF generation when big
# figures are involved.
#
# Call 'make pdf' for direct compilation to PDF using pdfTeX. Note that this
# requires you to use .pdf files. pdfTeX can not use .ps or .eps graphics.
# use epstopdf to convert such files to .pdf files.
#
#----------------------------------------------------------------------------
#adjust the following for your purpose

#set the a .dvi name that corresponds to your main .tex file
DVIFILES = template.dvi
MAINTEXFILE = $(DVIFILES:.dvi=.tex)
SUBTEXFILES = 
BIBFILES = template.bib

#switch = to # when using ps2pdf in win32 (mingw/msys), i.e. uncomment 2nd line
#E=\=
E=\#

#adjust paper size: letter/a4
PAPERSIZE=letter
PDFLATEXPAPERSIZE="-sPAPERSIZE$E$(PAPERSIZE)"
DVIPSPAPERSIZE=-t $(PAPERSIZE)
#uncomment the following two lines when using option tvcgpapersize
#DVIPSPAPERSIZE=-T 7.875in,10.75in
#PDFLATEXPAPERSIZE=

#----------------------------------------------------------------------------
LATEX = latex
BIBTEX = bibtex
L2H = latex2html
PDFLATEX = ps2pdf
PDFTEX = pdflatex
DVIPS = dvips 

RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined" 

PSFILES  = $(DVIFILES:.dvi=.ps) 

PDFFILES7 = $(DVIFILES:.dvi=.pdf7) 
PDFFILES8 = $(DVIFILES:.dvi=.pdf8) 

PDFTEXFILES = $(DVIFILES:.dvi=.pdftex)

COPY = if test -r $*.toc; then cp $*.toc $*.toc.bak; fi 
#RM = /usr/bin/rm -f 
RM = rm -f 

all:	msg gs8

msg:
	@echo "  This script defaults to GhostScript 8.  If you are using GhostScipt 7 please type"
	@echo "  make gs7 instead.  If unsure type gs -v from the command line"
	@echo "  To use pdflatex/pdftex, type make pdf"
	@echo ""


pdf:     clean pdftex 

gs7:        clean dvi ps pdf7

gs8:        clean dvi ps pdf8

dvi:           $(DVIFILES)

ps:           $(PSFILES)

pdf7:           $(PDFFILES7)

pdf8:           $(PDFFILES8)

pdftex:         $(PDFTEXFILES)

$(MAINTEXFILE) : $(SUBTEXFILES) $(BIBFILES)

%.dvi:			%.tex
				$(COPY);$(LATEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(LATEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.pdftex:			%.tex
				echo "wir sind da"
				$(COPY);$(PDFTEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(PDFTEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.ps:			%.dvi
#				dvips -T 7.875in,10.75in -Ppdf -G0 $< -o $@  #use tvcgpapersize
#				dvips -Ppdf -G0 $< -o $@
				dvips $(DVIPSPAPERSIZE) -Pdownload35 -Ppdf -G0 $< -o $@
#				dvips $< -o $@


%.pdf7:			%.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dMaxSubsetPct$E100" \
	"-dCompatibilityLevel$E1.3" \
	"-dSubsetFonts$Etrue" \
	"-dEmbedAllFonts$Etrue" \
	"-dAutoFilterColorImages$Efalse" \
	"-dAutoFilterGrayImages$Efalse" \
	"-dColorImageFilter$E/FlateEncode" \
	"-dGrayImageFilter$E/FlateEncode" \
	"-dMonoImageFilter$E/FlateEncode" \
	$< template.pdf

#				$(PDFLATEX) $<

%.pdf8:                 %.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dPDFSETTINGS=/prepress" \
	"-dCompatibilityLevel=1.3" \
	"-dAutoFilterColorImages=false" \
	"-dAutoFilterGrayImages=false" \
	"-dColorImageFilter=/FlateEncode" \
	"-dGrayImageFilter=/FlateEncode" \
	"-dMonoImageFilter=/FlateEncode" \
	"-dDownsampleGrayImages=false" \
	"-dDownsampleColorImages=false" \
	$< template.pdf
#                               $(PDFLATEX) $<

# cleans anything that can be re-generated automatically, plus emacs backups
clean: 
				rm -f *.aux *.log *.bbl *.blg *.brf *.cb *.ind *.idx *.ilg	\
				*.inx *.toc *.out $(DVIFILES) $(PSFILES) template.pdf *~

.PHONY : all pdf ps dvi clean $(MAINTEXFILE)


==> relatedwork-0318-1736.tex <==
\section{Related Work}
A large number of tools and studies exist for visualizations and analysis of tabular data. Our literature review lay the emphasis on two critical aspects, tabular data transformations and tabular visualizations.

\subsection{Tabular Data Transformation}

% For tabular data transformations, the purpose of most of the related works is to transform spreadsheets with arbitrary forms into a relational database schema. These works aim at removing hierarchical structures and redundant information from the spreadsheets to facilitate importing them into a database or other data tools. We broadly divide these studies into two categories, those that are non-automatic and require user involvement and those that are automatic and require no human intervention. Among these previous works, most of them are performed through non-automated methods. However, with the increasing scale of data, the efficiency of non-automated methods can hardly meet the demand. At the same time, technological advances have led to the improvement of computing power and the innovation of machine learning algorithms, making people's research gradually shift toward automation.

% (VERSION2) Most research studies about tabular data transformations is to transform tabular data with arbitrary forms into a relational database schema. These works aim at removing hierarchical structures and redundant information from the spreadsheets to facilitate importing them into a database or other data tools. 
% We broadly divide these studies into two categories, those that are non-automatic and require user involvement and those that are automatic and require no human intervention. Among these previous works, most of them are performed through non-automated methods. However, with the increasing scale of data, the efficiency of non-automated methods can hardly meet the demand. At the same time, technological advances have led to the improvement of computing power and the innovation of machine learning algorithms, making people's research gradually shift toward automation.
Most research studies about tabular data transformation rearrange the tabular data with arbitrary forms into a relational schema. These transformations remove the hierarchical structures and redundant information from tables and enable users to import the transformation results into the database or other data tools. 
We divide these studies into two categories, automatic and non-automatic approaches. The difference is that non-automatic techniques require users' involvement and automatic techniques do not. 


% Among the non-automated transformation methods, some require direct user programming to define transformation rules explicitly. Ajax~\cite{2000-AJAX-Galhardas} is a descriptive declarative language based on SQL statements that supports performing four transformations. Hung et al.~\cite{2011-spreadsheet-hung} propose TranSheet, a spreadsheet-like formula language that supports the user to perform five value-related transformations and six structure-related transformations. TabbyXL~\cite{2019-TabbyXL-Alexey} supports users to define functional and structural relationships of tables by using the domain-specific language CRL. These approaches are highly flexible, but learning these new languages to describe the transformation is difficult and time-consuming for the user. 
% (VERSION2) Some non-automated transformation methods require users to define transformation rules explicitly by low-level programming. Ajax~\cite{2000-AJAX-Galhardas} is a declarative language based on SQL statements that supports performing four transformations. TranSheet~\cite{2011-spreadsheet-hung} is a spreadsheet-like formula language that allow users to perform five value-related and six structure-related transformations. TabbyXL~\cite{2019-TabbyXL-Alexey} supports users to define functional and structural relationships of tables by using the domain-specific language. These approaches are highly flexible, but learning these new languages to describe the transformation is difficult and time-consuming for the user. \lgz{what is the relationship between Ajax, Transsheet, and TabbyXL}
% Most studies are about the non-automated transformation methods, which require users to define transformation rules explicitly. 
Among the non-automated transformation methods, some studies require user to define transformation rules explicitly by low-level programming. Ajax~\cite{2000-AJAX-Galhardas} is a declarative language based on SQL statements that supports four transformations. \lgz{detail transformations method} TranSheet~\cite{2011-spreadsheet-hung} is a spreadsheet-like formula language with better expressiveness that allows users to perform five value-related and six structure-related transformations. 
TabbyXL~\cite{2019-TabbyXL-Alexey} allows users to define functional and structural relationships of tables by using the domain-specific language. These approaches are highly flexible, but learning new syntax about data transformation is both difficult and time-consuming for users. \lgz{what is the relationship between Ajax, Transsheet, and TabbyXL}

% (VERSION1) Other works support users to transform the tabular data through interaction. Potter's Wheel~\cite{2001-PotterWheel-Raman} design a descriptive transformation language that allows users to perform their desired transformations by clicking on the menu bar. Wrangler~\cite{2011-Wrangler-Sean} extends the transformation language and adds a recommendation engine, where regular expressions can be generated based on user interaction to recommend subsequent transforming operations. The above two works do not take complex spreadsheets with hierarchical structures into consideration, while Xtable~\cite{1996-xtable-wang} supports modeling these hierarchical tables and performing a simple transformation on table headers. However, it does not consider the hierarchical relationships among data values.

In addition to the programming technique, some work allows users to transform tabular data interactively. 
Potter's Wheel~\cite{2001-PotterWheel-Raman} provides an interactive user interface based on a declarative grammar and allows users to perform their desired transformations by clicking on different menu bars. 
% \lgz{what is the difference between Potter's Wheel and programming method, provide a user interface based on the declarative language?} 
Furthermore, Wrangler~\cite{2011-Wrangler-Sean} extends the transformation language with a recommendation engine to generate regular expressions, which infers subsequent transforming operations based on user interactions. 
However, the above two studies do not take hierarchical tables into consideration. Xtable~\cite{1996-xtable-wang} builds an abstract model for hierarchical tables and provides an interactive environment for editing their logical structures. However, \lgz{it is not designed for the tabular data transformations and does not pay attention to the hierarchical relationships among data values.} \lgz{what is the ``hierarchical relationships among data values''?}


% As for the other kinds of studies targeting automatic transformations, some use the idea of example-oriented programming, where users can give some initial and final states in pairs as examples. The transformations required by users are described through a designed language. Also, a program is automatically generated by a designed algorithm, implementing the same transformations on subsequent inputs as described in the example pair. Gulwani et al. propose ProgFromEx~\cite{2011-Spreadsheet-Harris}, an algorithm that uses filter or associative program to infer the desired automatic transformation program. They also define a DAG-based algorithm in~\cite{2012-Spreadsheet-Gulwani}, which uses a \emph{generate and intersect} strategy for all programs that match the example and infers the final program through the defined ranking rules. Foofah\cite{2017-Foofah-Jin} constructs state diagrams based on user-supplied examples, representing all possible paths from the initial to the final state. A heuristic graph search algorithm is used to infer the best transformation program, with a pruning strategy to improve the search efficiency. Unlike the above works, which use whole tables as examples, Flashrelate~\cite{2015-FlashRelate-Barowy} requires only some tuples, including positive examples representing the desired transformations and negative examples representing the incorrect transformations. 



\lgz{Each section should begin with a summary sentence. Explain the relationships between different techniques. }

% We divide the automatic transformation techniques into three categories, example-oriented transformation, relational schema extraction, and machine-learning based methods. 
To improve the efficiency of tabular data transformations, some work focuses on the automatic transformation techniques. We divide these techniques into three categories, relational schema extraction, example-oriented transformation, and machine-learning based methods. 

The techniques based on the relational schema extraction identify and extract relational schema from original tables explicitly and transform them into canonical relational tables automatically. 
These studies explore different heuristic extraction algorithms based on domain knowledge. 
Cunha et al.~\cite{2009-database-cunha} construct relational patterns by extracting functional dependencies of spreadsheets.
Shigarov~\cite{2015-table-shigarov} and Su et al.~\cite{2017-Transforming-Su} acquire relational schema based on table boundary features and layout features.
In contrast, Dou et al.~\cite{2018-Expandable-Dou} obtain an extensible group representing the generic structure of the table by checking the formatting similarity and semantic similarity between cells. 
Paramonov et al.~\cite{2019-Heuristic-Viacheslav} modify the physical structure of the table header to make it more consistent with its hierarchical logical structure based on the text alignment and border characteristics within the cells to facilitate user understanding. 

Different with the techniques about relational schema extraction, example-oriented transformations do not define the relational schema explicitly.
Users only need to provide the initial and final states in pairs as an example and these techniques will generate a program automatically by implementing the same transformations as described in the example pairs.
ProgFromEx~\cite{2011-Spreadsheet-Harris} is an algorithm that uses filtering or associative program to infer the desired transformations. 
Based on ProgFromEx, a DAG-based algorithm~\cite{2012-Spreadsheet-Gulwani} uses a \emph{generate} and \emph{intersect} strategy for all programs that match the example and infers the final program through the defined ranking rules.
Foofah~\cite{2017-Foofah-Jin} constructs state diagrams based on user-supplied examples, representing all possible paths from the initial to the final state. 
It uses a heuristic graph search algorithm to infer the best transformation, with a pruning strategy to improve the searching efficiency. 
To reduce the difficulty of building example pair, Flashrelate~\cite{2015-FlashRelate-Barowy} requires only some tuples as examples instead of the whole table, including positive examples representing the desired transformations and negative examples representing the incorrect transformations. 

% Other work automatically identify and extract relational schema in original tables and transform those with arbitrary formats into canonical relational data tables. These works can be broadly classified into two categories, one of which manually designs algorithms through heuristic information such as domain knowledge. Cunha et al.~\cite{2009-database-cunha} construct relational patterns by extracting functional dependencies of spreadsheets but do not consider complex tables with a hierarchical structure. Shigarov~\cite{2015-table-shigarov} and Su et al.~\cite{2017-Transforming-Su} acquire relational schema based on table boundary features and layout features. In contrast, Dou et al.~\cite{2018-Expandable-Dou} obtain an extensible group representing the generic structure of the table by checking the formatting similarity and semantic similarity between cells. Based on the obtained results, the table can be transformed. Paramonov et al.~\cite{2019-Heuristic-Viacheslav} modify the physical structure of the table header to make it more consistent with its hierarchical logical structure based on the text alignment and border characteristics within the cells, aiding user understanding. 

\lgz{the relationships between the following research work}
The example-oriented algorithms infer tabular data transformation process explicitly based on the example pairs provided by users.  
In addition, many research studies explore the machine learning techniques for tabular data transformations.  
Chen et al.~\cite{2013-Automatic-Chen} use conditional random fields (CRF) to identify the hierarchical structure of table headers and generate relational tuples for each data automatically. 
Chen et al.~\cite{2017-Spreadsheet-chen} combine an active learning framework with user-supplied rules to build a spreadsheet attribute monitor. 
Dong et al.~\cite{2019-semantic-dong} apply multi-task learning method for form detection, header recognition, and cell classification problems.
TabularNet~\cite{2021-TabularNet-Du} constructed a neural network structure, which focuses on spatial location information and associative relationship information of tables.
Ghasemi-Gol et al.~\cite{2021-Learning-Majid} use a deep neural network model to embed the semantic and contextual information of cells and construct a model based on a recurrent neural network to classify the cells.


% Another type of work uses machine learning to generate transformation algorithms automatically. Chen et al.~\cite{2013-Automatic-Chen} use conditional random fields (CRF) to automatically identify the hierarchical structure of table headers and generate relational tuples for each data. Chen et al.~\cite{2017-Spreadsheet-chen} combine an active learning framework with user-supplied rules to build a spreadsheet attribute monitor. Dong et al.~\cite{2019-semantic-dong} simultaneously use multi-task learning ideas to consider form detection, header recognition, and cell classification problems. It uses the BERT language model to obtain semantic information of cells. Du et al.~\cite{2021-TabularNet-Du} constructed a neural network structure TabularNet, which focuses on spatial location information and associative relationship information of tables. Ghasemi-Gol et al.~\cite{2021-Learning-Majid} use a deep neural network model to embed the semantic and contextual information of cells and construct a model based on a recurrent neural network to classify the cells. To sum up, spreadsheets can be easily transformed into relational tables based on these machine-learning results.


\lgz{also missing the summary sentence at the beginning}
% The above works are relevant to us in the process of data transformations, but their starting points and purposes are not the same as ours.\lgz{more direct, what is the difference?}
% These works view the original spreadsheet as a form for merely displaying or storing data, and the purpose of transforming operations is to make spreadsheets formalized and easy to be imported into other data analysis tools. On the contrary, we use the spreadsheet itself as a tool for data analysis. Therefore, the data transformations we carry out are task-oriented. Users can select proper transforming operations based on their specific purpose so that the transformation results can more effectively assist the user in understanding the data. In addition, the transformations mentioned above involving complex tables with a hierarchical structure are one-way, i.e., they can only transform from complex tables to simple tables and not the other way around. Also, they do not support the transformation of the complex tables themselves.

The above research studies regard the tabular data as a data format and the goal is  to formalize their tabular structure to import into databases or other data analysis tools. 
However, HiTailor presents table as an interface for data analysis and presentation.
Therefore, the data transformations are task-oriented. Users determine the operations based on their specific purpose to assist users in understanding the data from different viewpoints. 
In addition, these methods also do not support the transformation of the hierarchical tables.
% In addition, the transformations mentioned above involves complex tables with a hierarchical structure are one-way, i.e., they can only transform from complex tables to simple tables and not the other way around. Also, they do not support the transformation of the complex tables themselves



% The above works are relevant to us in the process of data transformations, but their starting points and purposes are not the same as ours.\lgz{more direct, what is the difference?}
% These works view the original spreadsheet as a form for merely displaying or storing data, and the purpose of transforming operations is to make spreadsheets formalized and easy to be imported into other data analysis tools. On the contrary, we use the spreadsheet itself as a tool for data analysis. Therefore, the data transformations we carry out are task-oriented. Users can select proper transforming operations based on their specific purpose so that the transformation results can more effectively assist the user in understanding the data. In addition, the transformations mentioned above involving complex tables with a hierarchical structure are one-way, i.e., they can only transform from complex tables to simple tables and not the other way around. Also, they do not support the transformation of the complex tables themselves.

\subsection{Tabular Visualization}
% For table visualization, we focus on works related to \emph{visualization spreadsheets}~\cite{1997-spreadsheet-chi, 1998-Principles-Chi} or \emph{spreadsheet-like interfaces}~\cite{2001-Visualization-Jankun}. Their common feature is to embed different visual forms in each cell based on the original table structure. We broadly divide these works into two categories, one of which focuses on visualizations within a single table, and the other explores the connections between visualizing multiple tables.
\lgz{the differences between spreadsheet and table. the structure should be more clear. Single table-> keep individual cell, aggregate multiple cells, and build connections among multiple tables. }
For table visualization, we focus on works related to \emph{visualization spreadsheets}~\cite{1997-spreadsheet-chi, 1998-Principles-Chi} or \emph{spreadsheet-like interfaces}~\cite{2001-Visualization-Jankun}. Their common feature is to embed different visual forms in each cell with retaining the tabular layout structure. We divide these work into two categories, one of which focuses on visualizations within a single table, and the other explores the connections between visualizing multiple tables.

Among the studies about visualizing a single table, some only change the visual form within each cell without changing the original layout of the table. Table Lens~\cite{1994-table-rao} explores large data tables using a \emph{focus+context} mechanism to encode cell values based on the data types of different columns. It supports compression of row widths interactively in order to display more data. On this basis, FOCUS~\cite{1996-focus-spenke} combines interactive dynamic incremental database queries to filter the displayed data. It also allows users to merge identical adjacent values to increase readability. Taggle supports hierarchical aggregation and sorting for large tables with multiple columns, allowing the user to choose the appropriate visual form for the aggregated results. After Jacques Bertin proposed a matrix analysis method for tabular data,many works such as CHART~\cite{1977-interactive-benson} and Reorderable Matrix~\cite{2005-constructing-harri} applied it to computers, embedding visual forms to each cell in rows or columns. They also support the reordering of cell matrices to create spatial associations between similar cells. On top of that, Bertifier~\cite{2014-Revisiting-charles} achieves a significant increase in functionality and interactivity, facilitating the user to divide and annotate matrices into meaningful groups. There are also works that represent the table matrix as a Heatmap, which encodes the tabular data with different colors, such as ComplexHeatmaps~\cite{2016-heatmap-gu}. In addition to the above visualization tools for deterministic tabular data, Fuzzy Spreadsheet~\cite{2021-fuzzy-dhanoa} helps users track and explore uncertainty information, such as likelihood and probability distributions, to facilitate assumption analysis. 

Other work supports changes in the layout of relative positions between different columns. ValueCharts\cite{2004-ValueCharts-Carenini, 2006-integrated-bautista} addresses the multi-attribute ranking problem by encoding the visual form of each column according to user-assigned weights and then merging them to form a stacked bar chart. LineUp~\cite{2013-Lineup-Gratzl} enhances the flexibility of interaction based on this. It also establishes connections between stacked bars formed by user-specified weights and integrates them into a slope graph, facilitating users to compare multiple rankings of the same set of items. Podium~\cite{2017-podium-wall}, another type of multi-attribute ranking visualization tool, differs from the previous two works in that it collects users' perceptions and preferences of the data to invert the appropriate attribute weights.

In another type of work exploring connections between multiple tables, some try to establish connections between different subsets of data. For example, Domino~\cite{2014-Domino-Gratzl} chooses appropriate visualizations for each table within a data set, connecting multiple subsets in various ways to show the relationships between them. Other works focus on comparing different tables in a visual way, such as TACO~\cite{2018-TACO-Niederer}, which allows users to compare differences between multiple versions of the same table at different levels of granularity in an interactive way.

However, none of the aforementioned works takes the structure of tables with complex headers into consideration and simply apply the visual encoding directly to the same row or column, ignoring the possible hierarchical relationships between them. In addition, these works do not attempt to aggregate a part of the table to generate a single visualization form without changing the layout of cells.

==> relatedwork-20220319.tex <==
\section{Related Work}
A large number of tools and studies exist for visualizations and analysis of tabular data. Our literature review lay the emphasis on two critical aspects, tabular data transformations and tabular visualizations.

\subsection{Tabular Data Transformation}

% For tabular data transformations, the purpose of most of the related works is to transform spreadsheets with arbitrary forms into a relational database schema. These works aim at removing hierarchical structures and redundant information from the spreadsheets to facilitate importing them into a database or other data tools. We broadly divide these studies into two categories, those that are non-automatic and require user involvement and those that are automatic and require no human intervention. Among these previous works, most of them are performed through non-automated methods. However, with the increasing scale of data, the efficiency of non-automated methods can hardly meet the demand. At the same time, technological advances have led to the improvement of computing power and the innovation of machine learning algorithms, making people's research gradually shift toward automation.

% (VERSION2) Most research studies about tabular data transformations is to transform tabular data with arbitrary forms into a relational database schema. These works aim at removing hierarchical structures and redundant information from the spreadsheets to facilitate importing them into a database or other data tools. 
% We broadly divide these studies into two categories, those that are non-automatic and require user involvement and those that are automatic and require no human intervention. Among these previous works, most of them are performed through non-automated methods. However, with the increasing scale of data, the efficiency of non-automated methods can hardly meet the demand. At the same time, technological advances have led to the improvement of computing power and the innovation of machine learning algorithms, making people's research gradually shift toward automation.
Most research studies about tabular data transformation rearrange the tabular data with arbitrary forms into a relational schema. These transformations remove the hierarchical structures and redundant information from tables and enable users to import the transformation results into the database or other data tools. 
We divide these studies into two categories, automatic and non-automatic approaches. The difference is that non-automatic techniques require users' involvement and automatic techniques do not. 


% Among the non-automated transformation methods, some require direct user programming to define transformation rules explicitly. Ajax~\cite{2000-AJAX-Galhardas} is a descriptive declarative language based on SQL statements that supports performing four transformations. Hung et al.~\cite{2011-spreadsheet-hung} propose TranSheet, a spreadsheet-like formula language that supports the user to perform five value-related transformations and six structure-related transformations. TabbyXL~\cite{2019-TabbyXL-Alexey} supports users to define functional and structural relationships of tables by using the domain-specific language CRL. These approaches are highly flexible, but learning these new languages to describe the transformation is difficult and time-consuming for the user. 
% (VERSION2) Some non-automated transformation methods require users to define transformation rules explicitly by low-level programming. Ajax~\cite{2000-AJAX-Galhardas} is a declarative language based on SQL statements that supports performing four transformations. TranSheet~\cite{2011-spreadsheet-hung} is a spreadsheet-like formula language that allow users to perform five value-related and six structure-related transformations. TabbyXL~\cite{2019-TabbyXL-Alexey} supports users to define functional and structural relationships of tables by using the domain-specific language. These approaches are highly flexible, but learning these new languages to describe the transformation is difficult and time-consuming for the user. \lgz{what is the relationship between Ajax, Transsheet, and TabbyXL}
% Most studies are about the non-automated transformation methods, which require users to define transformation rules explicitly. 
Among the non-automated transformation methods, some studies require user to define transformation rules explicitly by low-level programming. Ajax~\cite{2000-AJAX-Galhardas} is a declarative language based on SQL statements that supports four transformations. \lgz{detail transformations method} TranSheet~\cite{2011-spreadsheet-hung} is a spreadsheet-like formula language with better expressiveness that allows users to perform five value-related and six structure-related transformations. 
TabbyXL~\cite{2019-TabbyXL-Alexey} allows users to define functional and structural relationships of tables by using the domain-specific language. These approaches are highly flexible, but learning new syntax about data transformation is both difficult and time-consuming for users. \lgz{what is the relationship between Ajax, Transsheet, and TabbyXL}

% (VERSION1) Other works support users to transform the tabular data through interaction. Potter's Wheel~\cite{2001-PotterWheel-Raman} design a descriptive transformation language that allows users to perform their desired transformations by clicking on the menu bar. Wrangler~\cite{2011-Wrangler-Sean} extends the transformation language and adds a recommendation engine, where regular expressions can be generated based on user interaction to recommend subsequent transforming operations. The above two works do not take complex spreadsheets with hierarchical structures into consideration, while Xtable~\cite{1996-xtable-wang} supports modeling these hierarchical tables and performing a simple transformation on table headers. However, it does not consider the hierarchical relationships among data values.

In addition to the programming technique, some work allows users to transform tabular data interactively. 
Potter's Wheel~\cite{2001-PotterWheel-Raman} provides an interactive user interface based on a declarative grammar and allows users to perform their desired transformations by clicking on different menu bars. 
% \lgz{what is the difference between Potter's Wheel and programming method, provide a user interface based on the declarative language?} 
Furthermore, Wrangler~\cite{2011-Wrangler-Sean} extends the transformation language with a recommendation engine to generate regular expressions, which infers subsequent transforming operations based on user interactions. 
However, the above two studies do not take hierarchical tables into consideration. Xtable~\cite{1996-xtable-wang} builds an abstract model for hierarchical tables and provides an interactive environment for editing their logical structures. However, \lgz{it is not designed for the tabular data transformations and does not pay attention to the hierarchical relationships among data values.} \lgz{what is the ``hierarchical relationships among data values''?}


% As for the other kinds of studies targeting automatic transformations, some use the idea of example-oriented programming, where users can give some initial and final states in pairs as examples. The transformations required by users are described through a designed language. Also, a program is automatically generated by a designed algorithm, implementing the same transformations on subsequent inputs as described in the example pair. Gulwani et al. propose ProgFromEx~\cite{2011-Spreadsheet-Harris}, an algorithm that uses filter or associative program to infer the desired automatic transformation program. They also define a DAG-based algorithm in~\cite{2012-Spreadsheet-Gulwani}, which uses a \emph{generate and intersect} strategy for all programs that match the example and infers the final program through the defined ranking rules. Foofah\cite{2017-Foofah-Jin} constructs state diagrams based on user-supplied examples, representing all possible paths from the initial to the final state. A heuristic graph search algorithm is used to infer the best transformation program, with a pruning strategy to improve the search efficiency. Unlike the above works, which use whole tables as examples, Flashrelate~\cite{2015-FlashRelate-Barowy} requires only some tuples, including positive examples representing the desired transformations and negative examples representing the incorrect transformations. 



\lgz{Each section should begin with a summary sentence. Explain the relationships between different techniques. }

% We divide the automatic transformation techniques into three categories, example-oriented transformation, relational schema extraction, and machine-learning based methods. 
To improve the efficiency of tabular data transformations, some research work focuses on the automatic transformation techniques. We divide these techniques into three categories, relational schema extraction, example-oriented transformation, and machine-learning based methods. 

The techniques based on the relational schema extraction identify and extract relational schema from the original tables explicitly and transform them into canonical relational tables automatically. 
These studies explore different heuristic extraction algorithms based on the domain knowledge. 
Cunha et al.~\cite{2009-database-cunha} construct relational patterns by extracting functional dependencies of spreadsheets.
Shigarov~\cite{2015-table-shigarov} and Su et al.~\cite{2017-Transforming-Su} acquire relational schema based on table boundary features and layout features.
In contrast, Dou et al.~\cite{2018-Expandable-Dou} obtain an extensible group representing the generic structure of the table by checking the formatting similarity and semantic similarity between cells. 
Paramonov et al.~\cite{2019-Heuristic-Viacheslav} modify the physical structure of the table header to make it more consistent with its hierarchical logical structure based on the text alignment and border characteristics within the cells to facilitate user understanding. 

Different with the techniques about relational schema extraction, the example-oriented transformations do not need to understand the explicit relational schema, but require users to provide initial and final states in pairs as an example. 
The example-oriented transformations generate a program automatically by implementing the same transformations as described in the example pairs. 
ProgFromEx~\cite{2011-Spreadsheet-Harris} is an algorithm that uses filtering or associative program to infer the desired transformations. 
Based on ProgFromEx, a DAG-based algorithm~\cite{2012-Spreadsheet-Gulwani} uses a \emph{generate} and \emph{intersect} strategy for all programs that match the example and infers the final program through the defined ranking rules.
Foofah\cite{2017-Foofah-Jin} constructs state diagrams based on user-supplied examples, representing all possible paths from the initial to the final state. 
It uses a heuristic graph search algorithm to infer the best transformation, with a pruning strategy to improve the searching efficiency. 
To reduce the difficulty of building example pair, Flashrelate~\cite{2015-FlashRelate-Barowy} requires only some tuples as examples instead of the whole table, including positive examples representing the desired transformations and negative examples representing the incorrect transformations. 

% Other work automatically identify and extract relational schema in original tables and transform those with arbitrary formats into canonical relational data tables. These works can be broadly classified into two categories, one of which manually designs algorithms through heuristic information such as domain knowledge. Cunha et al.~\cite{2009-database-cunha} construct relational patterns by extracting functional dependencies of spreadsheets but do not consider complex tables with a hierarchical structure. Shigarov~\cite{2015-table-shigarov} and Su et al.~\cite{2017-Transforming-Su} acquire relational schema based on table boundary features and layout features. In contrast, Dou et al.~\cite{2018-Expandable-Dou} obtain an extensible group representing the generic structure of the table by checking the formatting similarity and semantic similarity between cells. Based on the obtained results, the table can be transformed. Paramonov et al.~\cite{2019-Heuristic-Viacheslav} modify the physical structure of the table header to make it more consistent with its hierarchical logical structure based on the text alignment and border characteristics within the cells, aiding user understanding. 

\lgz{the relationships between the following research work}
Many research studies also explore the tabular data transformations based on different machine learning techniques.
Chen et al.~\cite{2013-Automatic-Chen} use conditional random fields (CRF) to identify the hierarchical structure of table headers and generate relational tuples for each data automatically. 
Chen et al.~\cite{2017-Spreadsheet-chen} combine an active learning framework with user-supplied rules to build a spreadsheet attribute monitor. 
Dong et al.~\cite{2019-semantic-dong} apply multi-task learning method for form detection, header recognition, and cell classification problems.
TabularNet~\cite{2021-TabularNet-Du} constructed a neural network structure, which focuses on spatial location information and associative relationship information of tables.
Ghasemi-Gol et al.~\cite{2021-Learning-Majid} use a deep neural network model to embed the semantic and contextual information of cells and construct a model based on a recurrent neural network to classify the cells.


% Another type of work uses machine learning to generate transformation algorithms automatically. Chen et al.~\cite{2013-Automatic-Chen} use conditional random fields (CRF) to automatically identify the hierarchical structure of table headers and generate relational tuples for each data. Chen et al.~\cite{2017-Spreadsheet-chen} combine an active learning framework with user-supplied rules to build a spreadsheet attribute monitor. Dong et al.~\cite{2019-semantic-dong} simultaneously use multi-task learning ideas to consider form detection, header recognition, and cell classification problems. It uses the BERT language model to obtain semantic information of cells. Du et al.~\cite{2021-TabularNet-Du} constructed a neural network structure TabularNet, which focuses on spatial location information and associative relationship information of tables. Ghasemi-Gol et al.~\cite{2021-Learning-Majid} use a deep neural network model to embed the semantic and contextual information of cells and construct a model based on a recurrent neural network to classify the cells. To sum up, spreadsheets can be easily transformed into relational tables based on these machine-learning results.


\lgz{also missing the summary sentence at the beginning}
% The above works are relevant to us in the process of data transformations, but their starting points and purposes are not the same as ours.\lgz{more direct, what is the difference?}
% These works view the original spreadsheet as a form for merely displaying or storing data, and the purpose of transforming operations is to make spreadsheets formalized and easy to be imported into other data analysis tools. On the contrary, we use the spreadsheet itself as a tool for data analysis. Therefore, the data transformations we carry out are task-oriented. Users can select proper transforming operations based on their specific purpose so that the transformation results can more effectively assist the user in understanding the data. In addition, the transformations mentioned above involving complex tables with a hierarchical structure are one-way, i.e., they can only transform from complex tables to simple tables and not the other way around. Also, they do not support the transformation of the complex tables themselves.

The above works are relevant to us in the process of data transformations, but their starting points and purposes are not the same as ours.\lgz{more direct, what is the difference?}
% These works view the original spreadsheet as a form for merely displaying or storing data, and the purpose of transforming operations is to make spreadsheets formalized and easy to be imported into other data analysis tools. On the contrary, we use the spreadsheet itself as a tool for data analysis. Therefore, the data transformations we carry out are task-oriented. Users can select proper transforming operations based on their specific purpose so that the transformation results can more effectively assist the user in understanding the data. In addition, the transformations mentioned above involving complex tables with a hierarchical structure are one-way, i.e., they can only transform from complex tables to simple tables and not the other way around. Also, they do not support the transformation of the complex tables themselves.

\subsection{Tabular Visualization}
% For table visualization, we focus on works related to \emph{visualization spreadsheets}~\cite{1997-spreadsheet-chi, 1998-Principles-Chi} or \emph{spreadsheet-like interfaces}~\cite{2001-Visualization-Jankun}. Their common feature is to embed different visual forms in each cell based on the original table structure. We broadly divide these works into two categories, one of which focuses on visualizations within a single table, and the other explores the connections between visualizing multiple tables.
\lgz{the differences between spreadsheet and table. the structure should be more clear. Single table-> keep individual cell, aggregate multiple cells, and build connections among multiple tables. }
For table visualization, we focus on works related to \emph{visualization spreadsheets}~\cite{1997-spreadsheet-chi, 1998-Principles-Chi} or \emph{spreadsheet-like interfaces}~\cite{2001-Visualization-Jankun}. Their common feature is to embed different visual forms in each cell with retaining the tabular layout structure. We divide these work into two categories, one of which focuses on visualizations within a single table, and the other explores the connections between visualizing multiple tables.

Among the studies about visualizing a single table, some only change the visual form within each cell without changing the original layout of the table. Table Lens~\cite{1994-table-rao} explores large data tables using a \emph{focus+context} mechanism to encode cell values based on the data types of different columns. It supports compression of row widths interactively in order to display more data. On this basis, FOCUS~\cite{1996-focus-spenke} combines interactive dynamic incremental database queries to filter the displayed data. It also allows users to merge identical adjacent values to increase readability. Taggle supports hierarchical aggregation and sorting for large tables with multiple columns, allowing the user to choose the appropriate visual form for the aggregated results. After Jacques Bertin proposed a matrix analysis method for tabular data,many works such as CHART~\cite{1977-interactive-benson} and Reorderable Matrix~\cite{2005-constructing-harri} applied it to computers, embedding visual forms to each cell in rows or columns. They also support the reordering of cell matrices to create spatial associations between similar cells. On top of that, Bertifier~\cite{2014-Revisiting-charles} achieves a significant increase in functionality and interactivity, facilitating the user to divide and annotate matrices into meaningful groups. There are also works that represent the table matrix as a Heatmap, which encodes the tabular data with different colors, such as ComplexHeatmaps~\cite{2016-heatmap-gu}. In addition to the above visualization tools for deterministic tabular data, Fuzzy Spreadsheet~\cite{2021-fuzzy-dhanoa} helps users track and explore uncertainty information, such as likelihood and probability distributions, to facilitate assumption analysis. 

Other work supports changes in the layout of relative positions between different columns. ValueCharts\cite{2004-ValueCharts-Carenini, 2006-integrated-bautista} addresses the multi-attribute ranking problem by encoding the visual form of each column according to user-assigned weights and then merging them to form a stacked bar chart. LineUp~\cite{2013-Lineup-Gratzl} enhances the flexibility of interaction based on this. It also establishes connections between stacked bars formed by user-specified weights and integrates them into a slope graph, facilitating users to compare multiple rankings of the same set of items. Podium~\cite{2017-podium-wall}, another type of multi-attribute ranking visualization tool, differs from the previous two works in that it collects users' perceptions and preferences of the data to invert the appropriate attribute weights.

In another type of work exploring connections between multiple tables, some try to establish connections between different subsets of data. For example, Domino~\cite{2014-Domino-Gratzl} chooses appropriate visualizations for each table within a data set, connecting multiple subsets in various ways to show the relationships between them. Other works focus on comparing different tables in a visual way, such as TACO~\cite{2018-TACO-Niederer}, which allows users to compare differences between multiple versions of the same table at different levels of granularity in an interactive way.

However, none of the aforementioned works takes the structure of tables with complex headers into consideration and simply apply the visual encoding directly to the same row or column, ignoring the possible hierarchical relationships between them. In addition, these works do not attempt to aggregate a part of the table to generate a single visualization form without changing the layout of cells.
